On-the-fly Vertex Reuse for Massively-Parallel Software Geometry Processing

Compute-mode rendering is becoming more and more attractive for non-standard rendering applications, due to the high flexibility of compute-mode execution. These newly designed pipelines often include streaming vertex and geometry processing stages. In typical triangle meshes, the same transformed vertex is on average required six times during rendering. To avoid redundant computation, a post-transform cache is traditionally suggested to enable reuse of vertex processing results. However, traditional caching neither scales well as the hardware becomes more parallel, nor can be efficiently implemented in a software design. We investigate alternative strategies to reusing vertex shading results on-the-fly for massively parallel software geometry processing. Forming static and dynamic batching on the data input stream, we analyze the effectiveness of identifying potential local reuse based on sorting, hashing, and efficient intra-thread-group communication. Altogether, we present four vertex reuse strategies, tailored to modern parallel architectures. Our simulations showcase that our batch-based strategies significantly outperform parallel caches in terms of reuse. On actual GPU hardware, our evaluation shows that our strategies not only lead to good reuse of processing results, but also boost performance by $2-3\times$ compared to na\"ively ignoring reuse in a variety of practical applications.

==> batchbuilder.tex <==
\begin{algorithm}
	\DontPrintSemicolon
	\SetKw{Sync}{syncthreads}
	\SetKw{To}{to}
	\SetKw{Shared}{shared}
	\SetKw{MaxBatchSize}{BatchSize}
	\SetKw{BlockSize}{BlockSize}
	\SetKw{Sort}{BitonicSort}
	\SetKw{PrefixSum}{PrefixSum}
	\SetKw{VertexShader}{shade}
	\SetKw{Tid}{tId}
	\SetKw{Output}{output}
	\SetKw{IIf}{if}
	\SetKw{IElse}{else}
	\SetKw{IThen}{then}
	\SetKw{Size}{size}
	\SetKw{Cas}{atomicCAS}
	\SetKw{Hash}{hash}
	\SetKw{Prob}{probing}
	\SetKw{push}{push}
	\SetKw{increase}{increasePriority}
	\SetKw{decrease}{decreasePriority}
	\SetKw{pop}{pop}
	\SetKw{app}{writeIndices}
	\SetKw{Or}{or}
	\SetKw{PQ}{PriorityQueue}
	\SetKw{CW}{VertexWeight}
	\SetKw{VW}{ValenceWeight}
	\SetKw{Target}{TargetBatchSize}

    %\Shared ids[\MaxBatchSize]\;
    %\Shared linIds[\MaxBatchSize]\;
    %\Shared mapped[\MaxBatchSize]\;
    %\Shared marks[\MaxBatchSize]\;
    %\Shared uniqueIds[\BlockSize]\;
    %\Shared v[\BlockSize]\;
    
   	$\VW \leftarrow 1$\;
   	$\CW \leftarrow 1000$\;
    
    \PQ $q$\;
    \For{$f \in faces$}{
    	 %$s \leftarrow$ sum over face vertex valences\;
    	 $s \leftarrow \sum_{v\in f} valence(v)$\;
    	 $\push(q,f,-s \cdot \VW)$\;
	}

	$V \leftarrow \emptyset$\;
	$B \leftarrow 0$\;
	\While{$q\neq \emptyset$}{
		$f \leftarrow \pop(q)$\;
	 	$\app(f)$\;
		$B \leftarrow B + |f|$\;
		\For{$v \in vertices(f)$}{
			\uIf{$v \notin V$}{
				$\Delta s = \VW + \CW$\; 
				$V \leftarrow \{V,v\}$\;
			}
			\Else{
				$\Delta s = \VW$\;
			}
			\For{$(f_n | v \in f_n)$}{
				\If{$f_n \in q$}{$\increase(q, f_n, \Delta s)$ }
			}
		}
		\If{$B = \Target$}{
			\For{$v \in V$}{
				\For{$(f_n | v \in f_n)$}{
					\If{$f_n \in q$}{$\decrease(q, f_n, \CW)$ }
				}	
			}
			$V \leftarrow \emptyset$\;
			$B \leftarrow 0$\;
		} 
	}

	\caption{Batching}
	\label{alg:batching}
\end{algorithm}
